Detecting Malicious Source Code in PyPI Packages with LLMs: Does RAG Come in Handy?

Malicious software packages in open-source ecosystems, such as PyPI, pose growing security risks. Unlike traditional vulnerabilities, these packages are intentionally designed to deceive users, making detection challenging due to evolving attack methods and the lack of structured datasets. In this work, we empirically evaluate the effectiveness of Large Language Models (LLMs), Retrieval-Augmented Generation (RAG), and few-shot learning for detecting malicious source code. We fine-tune LLMs on curated datasets and integrate YARA rules, GitHub Security Advisories, and malicious code snippets with the aim of enhancing classification accuracy. We came across a counterintuitive outcome: While RAG is expected to boost up the prediction performance, it fails in the performed evaluation, obtaining a mediocre accuracy. In contrast, few-shot learning is more effective as it significantly improves the detection of malicious code, achieving 97% accuracy and 95% balanced accuracy, outperforming traditional RAG approaches. Thus, future work should expand structured knowledge bases, refine retrieval models, and explore hybrid AI-driven cybersecurity solutions.

==> src/dataset.tex <==
\section{Evaluation}
\label{dataset}
The data in this research comes from the PyPI packages in the DataDog malicious software packages dataset \cite{OpenSourceDatasetMaliciousSoftwarePackages}, which contains over 1,929 packages identified as malicious from the Python ecosystem. These packages were processed using Python's Abstract Syntax Tree (AST) to extract relevant code behaviour features, such as system calls, file interactions, and sensitive operations. This feature extraction process offers a deeper analysis of the package behaviour than relying on metadata alone. Due to specific challenges such as escape codes and obfuscation in the code, some packages could not be processed. As a result, we successfully extracted features from 1,242 packages, while others were discarded due to parsing issues.

We used a pre-extracted source code from our professor for the benign dataset, which contained 139 malicious packages and 5193 benign packages. After applying the same AST-based feature extraction process, we extracted features \cite{zhang2023malicious} from 93 malicious and 3752 benign packages. These extracted features are then converted into textual descriptions that serve as the input for fine-tuning our large language models (LLMs). The features extracted from the packages, such as imports and system calls, are mapped to descriptive labels as shown in Table \ref{tab:feature-description}. These feature descriptions will help improve the model’s ability to detect malicious behaviour based on code operations rather than relying on metadata alone.


\begin{comment}
	

\begin{table}[ht]
    \centering
    \caption{Feature Descriptions for Package Behavior.}
    \begin{tabular}{|c|l|} \hline
    \label{tab:feature-description}
    \textbf{Feature Code} & \textbf{Feature Description} \\ \hline
        R1 & import operating system module \\ \hline
        R2 & use operating system module call \\ \hline
        R3 & import file system module \\ \hline
        R4 & use file system module file \\ \hline
        R5 & read sensitive information \\ \hline
        T1 & import network module \\ \hline
        T2 & use network module call \\ \hline
        T3 & use URL \\ \hline
        E1 & import encoding module \\ \hline
        E2 & use encoding module call \\ \hline
        E3 & use base64 string \\ \hline
        E4 & use long string \\ \hline
        P1 & import process module \\ \hline
        P2 & use process module call \\ \hline
        P3 & use bash script \\ \hline
        P4 & evaluate code at run-time \\ \hline
    \end{tabular}    
\end{table}
\end{comment}


Example of a Textual Description:
\textit{"start entry selfedgamestudy-5.59/setup.py, import process module, import operating system module, use process module call, end of entry."}.

These textual descriptions, derived from the extracted features, will be used as input for fine-tuning the LLMs, enabling the model to recognise malicious and benign code patterns based on their behaviour.




==> src/evaluation.tex <==
\section{Discussion}
\begin{enumerate}
    
    \item Strengths of your approach.
    \item Limitations (e.g., does it struggle with certain rule types?).
    \item Future improvements.
\end{enumerate}

==> src/futurework.tex <==
\section{Future Work}


==> src/threats.tex <==
\section{Threats to Validity}
\label{sec:threats}

Threats to \textit{internal validity} concern two aspects, \ie the literature analysis and the experiment design. Concerning the former, we acknowledge that we may miss relevant works in our review. To mitigate this, we followed well-established guidelines provided by \cite{ZHANG2011625} and searched the Scopus digital library that contain most of the peer-reviewed venues. Concerning the latter, the selected dataset can lead to biased results as it may not represent all possible malicious threats. In this respect, we leverage CRAG methodology combined with YARA rules to mitigate this issue.

\textit{External validity} is related to the generalizability of the whole approach, both in terms of programming languages and examined LLMs. Nevertheless, we considered three different configurations in the experiments by relying on a fine-tuning strategy that can be applied to different LLMs apart from the ones considered. Furthermore, the knowledge base used by CRAG can be customized and applied to additional programming languages.

==> src/xbackground.tex <==
\section{Background and Related Work}
\label{background}
This section provides an overview of current DC and DMA research. DMA is a decentralized approach to data management that enhances scalability by promoting domain-based ownership. While it enables faster growth and self-serve infrastructure, it creates challenges in maintaining consistent data quality and governance across domains. Solutions are needed to balance autonomy with standardized data practices. DC are an emerging solution for improving data quality in DMA environments by defining agreements between data producers and consumers. While they can reduce inconsistencies, most research lacks practical frameworks for automating and enforcing these DC in the real world. This paper presents an automated framework that uses DC to enforce data quality in a DMA. Integrating automated checks within the data pipeline supports decentralized ownership while ensuring compliance with governance standards, effectively tackling data quality challenges in DMA environments.
% \subsection{Smart Contract}

% The current research examines \textit{Smart Contracts}, which have recently garnered significant interest due to the rise of blockchain technology. Today, they are commonly understood as low-level code scripts operating on blockchains \cite{linklaters2017smart} \cite{clack2019smart}. 

% A smart contract is a self-executing digital contract where the terms of the agreement are encoded in computer code \cite{zou2019smart}. It automatically executes when specific conditions are met, facilitating, verifying, or enforcing the negotiation or performance of the contract. Smart contracts are primarily used in decentralized applications (DApps) and blockchain environments \cite{singh2023dapps}, and they are foundational to cryptocurrencies, decentralized finance (DeFi) \cite{aquilina2024decentralized}, and other blockchain applications. Typically written in programming languages like Solidity for the Ethereum blockchain \cite{lenarduzzi2018blockchain}, these contracts control assets, automate transactions, and enforce rules on a distributed ledger. They operate on a blockchain, and their execution is decentralized, often requiring network consensus for validation. 

\subsection{Data Contract and Data Quality}
A DC defines the standards for data quality, schema, and access between systems. It ensures data meets criteria before use and acts as an agreement between producers and consumers. HL Truong \cite{truong2011analyzing} introduces a model for DC in cloud-based data marketplaces, allowing for clear definitions of data rights, quality, and compliance. This framework supports standardized quality metrics such as accuracy and consistency, ensuring data meets specified standards. It enhances trust and usability in Data-as-a-Service (DaaS) environments. Florin-Bogdan\cite{balint2017supporting} introduce a platform for managing and monitoring DC within IoT dataspaces. The paper presents a contract-aware IoT platform that enables data flow monitoring. Using a microservice-based architecture and meta-model definitions, it verifies data compliance with contract terms as data flows through the system. Sun et al. \cite{sun2020contract} propose a contract-based resource-sharing method for scheduling tasks in fog-cloud environments. They leverage clusters of fog resources to enhance task execution, using a sealed-bid bilateral auction mechanism with buyers, sellers, and auctioneers. By analyzing betweenness centrality, computing performance, and communication delay, they identify optimal fog nodes, including mobile ones, within clusters. In this context, fog clusters can act as either buyers or sellers of node rights, with the cloud serving as a trusted intermediary for fog node auctions within specified time slots. Longo et al. \cite{longo2019cloud} emphasize the need for public contracts to adapt to changing public services, particularly data services. They argue that the rapid evolution of service requirements makes contracts "obsolete," calling for regular updates. To tackle this, they propose a cloud-based system to evaluate the Quality of Service (QoS) of Transportation Services in the Apulia Region, Southern Italy. This system manages contracts between service providers and the Regional Authority, using real-time data from passengers' smartphones to allow prompt adjustments to enhance QoS.

There is clearly limited research on DC, particularly regarding data quality, and none of the studies utilize a standard for DC eg. Open Data Contract Standard (ODCS) \cite{odcs}.





% Weiqin Zou \cite{zou2019smart} explores the current state of smart contract development, particularly in relation to blockchain technologies like Ethereum. It investigates developers' challenges when working with smart contracts and low-level code scripts executed on blockchain platforms.  Khan, Shafaq Naheed \cite{khan2021blockchain} presents a thorough overview of blockchain-enabled smart contracts from both technical and practical perspectives.
%  Gu, Yonggen in \cite{gu2018decentralized} proposed a decentralized transaction method using smart contracts and a VCG auction mechanism for efficient storage resource selection. Implemented on a private Ethereum chain, simulations show the model effectively addresses cost and availability issues. Daraghmi, Eman demonstrates 
%  in \cite{daraghmi2024smart} the use of Ethereum-based Quorum for smart contract deployment, offering a secure and transparent environment that allows for standardized smart contracts in a consortium framework, enabling third-party validation while maintaining privacy.

 \subsection{Data Mesh Architecture}
 DMA is a decentralized approach to data management that emphasizes ownership based on specific domains and treats data as a product \cite{dehghani2022data} \cite{bode2024towards}. In contrast to traditional centralized models, it encourages autonomous data management within individual domains, thereby enhancing scalability and agility. Current research investigates various aspects of DMA implementation, focusing on the technical challenges of creating autonomous, interoperable data domains and the sociotechnical implications of evolving data governance and ownership. Tom and Indika \cite{van2024architectural} present a list of architectural design choices and their options, including reviewed 43 industry articles about self-serve data platforms in DMA. Nemania and Damian \cite{borovits2023privacy} introduce a conceptual framework that integrates privacy engineering principles with the decentralized nature of DMA that offers a holistic perspective, capturing essential elements from both fields. It explores the intersections of privacy engineering and DMA dimensions and provides guidelines for stakeholders involved in a DMA initiative to enhance data privacy controls.
 CowMesh \cite{pakrashi2023cowmesh} describes a DMA designed for the dairy industry that focuses on facilitating access to data from farms in a decentralized fashion. Jan Bode \cite{bode2024towards}  offers insights into DMA adoption, highlighting motivations, challenges, and strategies from industry experts. It guides organizations aiming to decentralize data ownership and governance to enhance scalability, data quality, and accessibility. Data quality can improve with DMA adoption, as decentralized ownership enables domain experts to enhance quality using their contextual knowledge.

The existing studies have analyzed DMA implementations, developed components for a self-serve platform, and created reference architectures for DMA. However, none have addressed data quality for each domain.
